Computational Approaches to Understanding Large Language Model Impact on Writing and Information Ecosystems

Large language models (LLMs) have shown significant potential to change how we write, communicate, and create, leading to rapid adoption across society. This dissertation examines how individuals and institutions are adapting to and engaging with this emerging technology through three research directions. First, I demonstrate how the institutional adoption of AI detectors introduces systematic biases, particularly disadvantaging writers of non-dominant language varieties, highlighting critical equity concerns in AI governance. Second, I present novel population-level algorithmic approaches that measure the increasing adoption of LLMs across writing domains, revealing consistent patterns of AI-assisted content in academic peer reviews, scientific publications, consumer complaints, corporate communications, job postings, and international organization press releases. Finally, I investigate LLMs' capability to provide feedback on research manuscripts through a large-scale empirical analysis, offering insights into their potential to support researchers who face barriers in accessing timely manuscript feedback, particularly early-career researchers and those from under-resourced settings.

==> 1_introduction.tex <==
\chapter{Introduction}



Large language models (LLMs) such as ChatGPT~\citep{ChatGPT} have rapidly transformed how individuals and institutions engage with writing. From students drafting essays to scientists composing research manuscripts and companies crafting press releases, LLMs are now deeply embedded in communication workflows across society. Within mere months of ChatGPT's launch in late 2022, these powerful systems attracted over 100 million users, making it one of the fastest-growing consumer applications in history~\citep{reuters-chatgpt-sets-record-fastest-growing-user-base,forbes-chatgpt-hits-100-million}. This wave of adoption brings both immense opportunity and significant societal challenges. While LLMs have the potential to democratize writing and lower barriers to entry~\citep{lee2022evaluating,chatgpt-pass-medical-exam,chatgpt-wharton-mba}, their rapid deployment also raises concerns around fairness~\citep{Liang2023GPTDA}, accountability, and epistemic integrity~\citep{liang2024monitoring}.

The challenge we face is not simply technological but fundamentally about understanding how these tools are reshaping our information ecosystems---the complex networks of content creation, evaluation, and dissemination that underpin knowledge production and communication. Despite extensive discourse and speculation about widespread LLM use in sectors as diverse as education~\cite{bearman2023discourses}, the sciences~\cite{van2023ai, messeri}, and global media~\cite{fake-news-66}, we lack systematic methods to measure the scale of such use or evaluate how the introduction of generated text is affecting institutional practices and societal communication patterns.

This dissertation develops computational approaches to study the impact of LLMs on writing and information ecosystems across institutional, disciplinary, and societal contexts. Rather than focusing solely on the technological capabilities of these models, this work examines their real-world impact through three interconnected research projects that collectively provide a comprehensive framework for understanding how LLMs are transforming human communication.

\textbf{Institutional responses can unintentionally create new barriers.} The first line of work investigates how institutional attempts to regulate LLM use can inadvertently create new forms of bias and exclusion. In particular, institutions have begun to adopt AI content detectors to flag potential misuse of LLMs. Yet these detectors may themselves be flawed. We show that widely used GPT detectors systematically misclassify writing by non-native English speakers as AI-generated, while native-written texts are correctly classified~\citep{Liang2023GPTDA}. Through controlled experiments and adversarial prompting, we demonstrate that these misclassifications stem from a detector bias toward constrained linguistic expressions, highlighting the need for fairness-aware detection systems. This work cautions against over-reliance on black-box detection tools in evaluative or educational settings, particularly where they may exacerbate linguistic discrimination.

\textbf{Measuring real-world LLM adoption at scale.} Given that individual-level detection remains unreliable and potentially biased, the second line of work proposes a new population-level framework---\textit{distributional GPT quantification}---for estimating the prevalence of LLM-modified content in large corpora~\citep{liang2024monitoring}. This method uses reference data and maximum likelihood estimation to efficiently quantify LLM usage without requiring ground-truth annotations for each instance. The approach is more than seven orders of magnitude more computationally efficient than existing detection methods while achieving superior accuracy under realistic distribution shifts. Applying this framework, we conduct a series of large-scale empirical studies. First, we examine peer reviews submitted to major AI conferences post-ChatGPT, finding that up to 16.9\% of reviews may be substantially modified by LLMs, with usage patterns concentrated near deadlines and among lower-confidence reviewers~\citep{liang2024monitoring}. Second, we analyze over one million scientific papers across \textit{arXiv}, \textit{bioRxiv}, and the \textit{Nature} portfolio, showing a steady rise in LLM-assisted writing, especially in computer science, with higher usage among frequent preprint authors and shorter papers~\citep{liang2024mapping}. Third, we extend this analysis to societal-scale writing domains---consumer complaints, corporate press releases, job postings, and UN communications---and find widespread LLM adoption across sectors, with up to 24\% of content LLM-modified in many of the domains~\citep{liang2025widespread}.

\textbf{Leveraging LLMs to bridge access gaps.} Beyond identifying risks and quantifying adoption, our third line of work explores how LLMs may help bridge access gaps in scientific communication. We develop an LLM-based feedback system using GPT-4 and evaluate it on over 4,800 manuscripts from both \textit{Nature} journals and the \textit{ICLR} conference~\citep{liang2024can}. We find that GPT-4's feedback overlaps with human reviewer comments at comparable rates to reviewer-reviewer agreement (30-39\% vs 28-35\%), especially on weaker submissions. In a prospective user study with 308 researchers from 110 institutions, a majority reported that the LLM-generated feedback was helpful and in many cases preferable to reviews they had previously received. While human expert feedback remains foundational to scientific rigor, LLM feedback can complement and expand access to critique, particularly for early-career researchers and scholars from under-resourced institutions.

Together, these studies offer a data-driven lens into the evolving dynamics between generative AI and human communication. The work demonstrates that LLMs are not merely tools for individual productivity enhancement, but forces that are systematically reshaping how information is created, evaluated, and disseminated across society. Methodologically, this thesis integrates natural language processing, statistical inference, and human-subject evaluation to develop scalable approaches for understanding human-AI interaction in real-world settings. Substantively, it addresses fairness in AI deployment, the measurement of real-world LLM influence, and the role of LLMs in reshaping knowledge production.


The computational approaches developed in this dissertation provide both methodological contributions and empirical insights with immediate practical implications for educational institutions designing academic integrity policies, publishers developing submission guidelines, and organizations considering LLM integration into their workflows. The societal relevance of this work is reflected in its coverage by over 300 media outlets worldwide, including \textit{Nature}, \textit{The New York Times}, \textit{Scientific American}, \textit{The Guardian}, and \textit{Fortune}. As LLMs become increasingly embedded in institutional and societal infrastructures, it is imperative to ensure that their integration advances equity, transparency, and epistemic robustness. The findings point toward a future where human and artificial intelligence collaborate in writing and information production, but one that requires thoughtful design to preserve diversity, authenticity, and equitable access. 

The remainder of this dissertation is organized as follows. Chapter~\ref{ch:gpt-detectors} presents the analysis of bias in GPT detectors and their implications for non-native English writers. Chapter~\ref{ch:monitoring} introduces the distributional quantification framework and applies it to academic peer review. Chapters~\ref{ch:scientific-papers} and~\ref{ch:widespread-adoption} extend this framework to scientific publishing and broader societal domains respectively. Chapter~\ref{ch:scientific-feedback} examines the potential for LLMs to provide useful scientific feedback. Finally, Chapter~\ref{ch:conclusion} synthesizes the findings, discusses broader implications, and outlines directions for future research.


==> 4.Society/Sections/0_Abstract.tex <==

The recent advances in large language models (LLMs) attracted significant public and policymaker interest in its adoption patterns.  In this paper, we systematically analyze LLM-assisted writing across four domains—consumer complaints, corporate communications, job postings, and international organization press releases—from January 2022 to September 2024. Our dataset includes 687,241 consumer complaints, 537,413 corporate press releases, 304.3 million job postings, and 15,919 United Nations (UN) press releases.
%
Using a robust population-level statistical framework, we find that LLM usage surged following the release of ChatGPT in November 2022. By late 2024, roughly 18\% of financial consumer complaint text appears to be LLM-assisted, with adoption patterns spread broadly across regions and slightly higher in urban areas. For corporate press releases, up to 24\% of the text is attributable to LLMs. In job postings, LLM-assisted writing accounts for just below 10\% in small firms, and is even more common among younger firms. UN press releases also reflect this trend, with nearly 14\% of content being generated or modified by LLMs.
% 
Although adoption climbed rapidly post-ChatGPT, growth appears to have stabilized by 2024, reflecting either saturation in LLM adoption or increasing subtlety of more advanced models. Our study shows the emergence of a new reality in which firms, consumers and even international organizations substantially rely on generative AI for communications. 

